Sequential One-Sided Hypothesis Testing of Markov Chains

We study the problem of sequentially testing whether a given stochastic process is generated by a known Markov chain. Formally, given access to a stream of random variables, we want to quickly determine whether this sequence is a trajectory of a Markov chain with a known transition matrix $P$ (null hypothesis) or not (composite alternative hypothesis). This problem naturally arises in many engineering problems. The main technical challenge is to develop a sequential testing scheme that adapts its sample size to the unknown alternative. Indeed, if we knew the alternative distribution (that is, the transition matrix) $Q$, a natural approach would be to use a generalization of Wald's sequential probability ratio test (SPRT). Building on this intuition, we propose and analyze a family of one-sided SPRT-type tests for our problem that use a data-driven estimator $\hat{Q}$. In particular, we show that if the deployed estimator admits a worst-case regret guarantee scaling as $\mathcal{O}\left( \log{t} \right)$, then the performance of our test asymptotically matches that of SPRT in the simple hypothesis testing case. In other words, our test automatically adapts to the unknown hardness of the problem, without any prior information. We end with a discussion of known Markov chain estimators with $\mathcal{O}\left( \log{t} \right)$ regret.

==> 20_problem.tex <==
\subsection{Problem Formulation}
We consider the problem of composite hypothesis testing: a tester is given a known Markov chain, represented by its transition matrix $\boldsymbol{P}\in\mc{M}^m_1$, and a trajectory  $X_1,X_2,\ldots$ drawn from an underlying Markov chain with dynamics $\boldsymbol{P_X}\in\mc{M}^m_1$. 
The tester must decide 
\begin{align*}
    H_0: \boldsymbol{P_X} = \boldsymbol{P}\text{\ \ \ vs \ \ \ \ } H_1: \boldsymbol{P_X} \neq \boldsymbol{P}. %p_X \neq p.
\end{align*}

 Note that this problem generalizes the classical binary hypothesis testing with i.i.d.\ observations: the composite nature of the alternative hypothesis generalizes \textit{simple} hypothesis testing, where the tester compares against another known distribution. Furthermore, the Markov observation assumption extends the i.i.d.\ case, where the transition matrices reduce to 
 degenerate matrices with all rows equal to $p$ for the known target distribution, and $p_X$ governing the i.i.d.\ samples.  

We work in the sequential setting, where at each time step $t=1,2,\ldots$ the tester may choose to either end the testing and declare a hypothesis or may request another sample, continuing the test.  In this setting, we aim to develop a test which correctly declares $H_1$, rejecting the null hypothesis $\boldsymbol{P}$, in as few samples as possible while controlling type-1 errors.  

\begin{definition}
A \textit{level-$\alpha$, power-one} test is a test which defines a stopping time, $\tau$ with the following guarantees:
\begin{align}
    \label{eq:promises}
    \P_{H_0}(\tau<\infty) \leq \alpha \text{ and } \P_{H_1}(\tau<\infty) = 1. 
\end{align}
\end{definition}
We will characterize the performance of our algorithms via bounds on $\E_{H_1}[\tau]$,  the expected number of samples required to correctly reject the null hypothesis.

\subsection{Related Work}
\label{subsec:related}
Related, but distinct, problem formulations have been studied in a wide variety of contexts.
The most important factor that sets our work apart from all these works is our formulation where 1) we consider samples that are not drawn iid  in time but are instead Markov, and 2) we remove any assumption on the true distribution under the alternative hypothesis. Much of prior work on Markov chain testing consider a variety of constraints such as being fully known as a simple hypothesis~\cite{phatarford1965markov, wald1945SPRT}, uniform~\cite{fawzi2022sequential}, 
a subset of alternatives~\cite{auss2020minimax,hoeffding1965asymptotically, li2014generalized, zhang2018generalmarkov}. Similarly, in \textit{identity testing} between Markov chains associated with a contrast function, $d$ and a tolerance $\epsilon$~\cite{daskalakis2018testing, cherapanamjeri2019symmetric, wolfer2020ergodic, wolfer2023geometric}, the null hypothesis $\boldsymbol{P_X}=\boldsymbol{P}$ is tested against \textit{only} the ``$\epsilon$-separated alternatives'' $\{\boldsymbol{P}_X: (\boldsymbol{P},\boldsymbol{P_X})>\epsilon\}$.  Motivated by applications in anomaly detection, our work deviates from this and removes any assumption, including $\epsilon$-distance, on the true distribution under the alternative hypothesis. Relaxing the requirement on the tester to accept the null hypothesis at a bounded time, frees our analysis to account for a strongly asymmetric treatment of type-1 versus type-2 errors while also allowing us to take advantage of a sequential test with a random stopping time.

Work in this area is generally done in the PAC setting, promising a correct declaration with high probability while studying sample complexity over different choices of the contrast function $d$ and for various assumptions on the structure of both $\boldsymbol{P}$ and $\boldsymbol{P_X}$.

We will give a non-exhaustive survey of several of these lines of study here to highlight the unique characteristics of our problem setting as well as the connection to prior work.

In the hypothesis testing literature, Markov chains are most commonly studied for \textit{simple} alternatives and fixed-length analysis: where the null hypothesis' Markov chain is tested against a fixed, known alternative chain. These works generally consider the interplay between bounds on both type 1 and type 2 errors. Sequential hypothesis testing of Markov chains was first studied in~\cite{phatarford1965markov}, which directly extended Wald's SPRT~\cite{wald1945SPRT} to dependent data for tests between two fixed hypotheses.   The authors in~\cite{fauss2020minimax} also consider fixed alternatives, but consider minimax performance over uncertainty regions around the alternatives.  And \cite{natarajan1985largedev, nakagawa1993converse, watanabe2017finite} all study theoretically attainable error rates, subject to various constraints. While these studies do not allow for a composite alternative hypothesis and focus on both types of error, our proposed algorithm is motivated and structured similarly to SPRT against a data-driven estimate of the true distribution. In fact, we will show that by carefully selecting the estimator, our proposed algorithm is able to asymptotically match that of SPRT in the simple hypothesis testing case.  

A related approach that does address composite alternatives is the \textit{generalized} likelihood ratio test (GLRT)~\cite{hoeffding1965asymptotically} which~\cite{li2014generalized} extended to a sequential test for i.i.d. data and~\cite{zhang2018generalmarkov} to a non-sequential Markov test.  Our work departs from these in the combination of the sequential and Markov settings and in the one-sided nature of our desired test, which we discuss further below.

Our problem formulation is also related to \textit{identity testing} associated with a contrast function, $d$, between Markov chains and a tolerance $\epsilon$~\cite{daskalakis2018testing, cherapanamjeri2019symmetric, wolfer2020ergodic, wolfer2023geometric}. In Markov chain identity testing, the null hypothesis $\boldsymbol{P_X}=\boldsymbol{P}$ is tested against \textit{only} the ``$\epsilon$-separated alternatives'' $\{\boldsymbol{P}_X: (\boldsymbol{P},\boldsymbol{P_X})>\epsilon\}$.  Work in this area is generally done in the PAC setting, promising a correct declaration with high probability while studying sample complexity over different choices of the contrast function $d$ and for various assumptions on the structure of both $\boldsymbol{P}$ and $\boldsymbol{P_X}$.  While this problem formulation closely resemble ours, the proposed solutions differ significantly. This problem was first studied in~\cite{daskalakis2018testing} for the case of symmetric Markov chains by reduction to an i.i.d. identity testing problem.  Their solution's dependence on hitting time was later relaxed in~\cite{cherapanamjeri2019symmetric} by means of a more elaborate reduction.  The requirement of symmetry was then relaxed in~\cite{wolfer2020ergodic}, in which the authors provide a test which only depends on ergodicity of the reference chain. More recently, information geometric approaches used in~\cite{wolfer2023geometric} offer novel, efficient proof techniques via embedding the problem in a larger state space to recover known bounds for reversible chains. 

The primary differences between our formulation and the identity testing papers above are the assumption of a given, fixed number of samples and knowledge of the separation $\epsilon$. While in the i.i.d case with a uniform distribution null hypothesis the authors in~\cite{fawzi2022sequential} have considered the advantages of sequential algorithms, to the best of our knowledge the sequential version of the Markov identity testing has not been studied. Furthermore, by considering a one-sided formulation, we remove any assumption, including $\epsilon$-distance, on the true distribution under the alternative hypothesis. In fact, the one-sided formulation is fundamentally different  from the other works discussed above where a strongly asymmetric treatment of type-1 versus type-2 errors is considered.  Without some guarantee as how far the true distribution under the alternative is from the null distribution, we instead relaxing the requirement on the tester to accept the null hypothesis to free our analysis of the need to characterize the worst-case alternative distribution which often complicates identity testing. To illustrate the advantages of sequential algorithms while accounting for the main differences introduced in the one-sided setting, we present simulations that compare our algorithm with an appropriately modified version of the fixed length test of~\cite{wolfer2020ergodic}.  Our simulation results in Section~\ref{subsec:adaptivity} illustrate this. 

%Comparing only to known alternative(s) is one way to resolve this challenge, allowing an uncertainty ball around the null hypothesis is another.  Given the anomaly detection framework that motivates our problem, we choose instead to address this by requiring the test run indefinitely under the null hypothesis and disallowing type 2 errors.  We will discuss some of the results of this distinction in the analysis below.     

%Finally, many existing works put stringent restrictions on the structure of either the reference Markov chain, the true data-generating chain, or both.  The only assumption made in this work is the existence of a stationary distribution for the data-generating chain.  

Further afield from our work is the broader topic of property testing, which is thoroughly covered by the survey~\cite{canonne2020survey}.  An important subset of this field is testing if data is generated from an arbitrary distribution with the Markov property~\cite{besag2013exact}, \cite{chen2012testing}.  While this can be used to reject the null, it does not address testing among multiple Markov chains where the alternative is also Markovian.  

% More relevant to our practical motivations, the topic of change detection covers a variety of methods intended to alert upon a change in the model generating a stream of data, see~\cite{Xie2021change} for a survey of related results.
